Interactive Steering of Hierarchical Clustering

Hierarchical clustering is an important technique to organize big data for exploratory data analysis. However, existing one-size-fits-all hierarchical clustering methods often fail to meet the diverse needs of different users. To address this challenge, we present an interactive steering method to visually supervise constrained hierarchical clustering by utilizing both public knowledge (e.g., Wikipedia) and private knowledge from users. The novelty of our approach includes 1) automatically constructing constraints for hierarchical clustering using knowledge (knowledge-driven) and intrinsic data distribution (data-driven), and 2) enabling the interactive steering of clustering through a visual interface (user-driven). Our method first maps each data item to the most relevant items in a knowledge base. An initial constraint tree is then extracted using the ant colony optimization algorithm. The algorithm balances the tree width and depth and covers the data items with high confidence. Given the constraint tree, the data items are hierarchically clustered using evolutionary Bayesian rose tree. To clearly convey the hierarchical clustering results, an uncertainty-aware tree visualization has been developed to enable users to quickly locate the most uncertain sub-hierarchies and interactively improve them. The quantitative evaluation and case study demonstrate that the proposed approach facilitates the building of customized clustering trees in an efficient and effective manner.

==> acknowledge.tex <==
\acknowledgments{
This research was funded by National Key R\&D Program of China (No.  2018YFB1004300), the National Natural Science Foundation of China (No.s 61761136020, 61672308), and Microsoft Research Asia.
% The authors would like to thank Liwang Zhou for implementing part of the learning-from-crowds algorithm and the anonymous reviewers for their valuable comments. B. Wang is the corresponding author.
\looseness=-1}

==> background.tex <==
\section{Constrained Clustering Algorithm}
\label{Alg.BRT}

In addition to the extracted constraints, the clustering results should also faithfully represent the original data distribution \textbf{(R1.2)}.
Given the constraint tree $T_c$, we next build a hierarchy $T$ for a document collection $D$.
According to Wang et al.~\cite{wang2013mining}, the constrained hierarchical clustering problem can be solved by maximizing the posterior probability of $T$
\begin{equation}
p(T\mid D, T_c) \propto p(D\mid T)p(T\mid T_c).
\label{eq:posterior}
\end{equation}
Here $p(D\mid T)$ represents how well $T$ fits the distribution of $D$ (data-driven) and $p(T\mid T_c)$ denotes how similar $T$ is to $T_c$ (knowledge-driven).

\noindent \textbf{Data-driven.} 
 The data-driven term $p(D\mid T)$ can be calculated in a recursive form:
$p(D\mid T)=\pi_{T} f(D)+(1-\pi_{T})\prod_{T_i\in\mathrm{children}(T)} p(D_i\mid T_i)$, 
where $\pi_{T}$ is the prior probability that all documents in $D$ are kept in one cluster, and $D_i$ represents the set of documents in sub-tree $T_i$.
The marginal probability $f(D)$ is defined by using the DCM distribution $f(D)=f_{DCM}(D)=\prod_{d_i\in D}f_{DCM}(d_i,D)$.


\noindent \textbf{Knowledge-driven.}
Similarly, for any given sub-hierarchy $T_m$, we define the knowledge-driven term $p(T_m\mid T_c)$ in a recursive form: $p(T_m\mid T_c)=p(T_i\mid T_c)p(T_j\mid T_c)p(T_m\mid T_i,T_j,T_c)$.
Here $T_i$ and $T_j$ are the sub-trees that are merged to generate $T_m$. $p(T_m\mid T_i,T_j,T_c)$ measures how many constraints are violated in the merging operation.
We consider the constraints as triples and fans, because Ng et al.~\cite{ng1996reconstruction} show that triples and fans can be used to uniquely define a hierarchy (i.e., contain all hierarchical information of $T_c$).
Specifically, for every three documents $d_a,d_b,d_c$, a triple $d_a d_b\mid d_c$ means that $d_a, d_b$ are merged before $d_c$ joins them, while a fan $(d_a, d_b, d_c)$ means that the three documents are merged simultaneously.
We may decompose $T_c$ into triples and fans and compute how many of them do not exist anymore in $T_m$.
Inspired by Markov Random Field (MRF), we define the violation term as
\begin{equation}
p(T_m\mid T_i,T_j, T_c)\overset{\Delta}{=}\frac{1}{Z}\exp\left(-\lambda V_{T_c}(\{T_i,T_j\}\rightarrow T_m)\right)\label{eq:Energy}.
\end{equation}
Here $V_{T_c}(\{T_i,T_j\}\rightarrow T_m)$ is the number of triples or fans that are violated when we merge $T_i$ and $T_j$ to generate $T_m$,
$Z$ is the normalizing constant,
and the constraint weight $\lambda$ balances the knowledge-driven term and the data-driven term.

\noindent \textbf{Optimization}.
We maximize Eq.~(\ref{eq:posterior}) by using a greedy agglomerative strategy~\cite{blundell2010bayesian}.
Initially, each document is treated as a sub-tree. 
At each iteration, the algorithm searches all candidate pairs of sub-trees and merges the pair with the highest posterior ratio


\begin{equation}
\frac{p(D_m\mid T_m)}{p(D_i\mid T_i)p(D_j\mid T_j)}\cdot\frac{p(T_m\mid T_c)}{p(T_i\mid T_c)p(T_j\mid T_c)}.
\label{eq:new_ratio}
\end{equation}
Here $D_i$, $D_j$, and $D_m$ are the document sets for $T_i$, $T_j$, and $T_m$, respectively. $T_m$ is the result of merging $T_i$ and $T_j$, and $D_m=D_i\cup D_j$.
